Controlled Text Generation with Natural Language Instructions

Large language models generate fluent texts and can follow natural language instructions to solve a wide range of tasks without task-specific training. Nevertheless, it is notoriously difficult to control their generation to satisfy the various constraints required by different applications. In this work, we present InstructCTG, a controlled text generation framework that incorporates different constraints by conditioning on natural language descriptions and demonstrations of the constraints. In particular, we first extract the underlying constraints of natural texts through a combination of off-the-shelf NLP tools and simple heuristics. We then verbalize the constraints into natural language instructions to form weakly supervised training data. By prepending natural language descriptions of the constraints and a few demonstrations, we fine-tune a pre-trained language model to incorporate various types of constraints. Compared to existing search-based or score-based methods, InstructCTG is more flexible to different constraint types and has a much smaller impact on the generation quality and speed because it does not modify the decoding procedure. Additionally, InstructCTG allows the model to adapt to new constraints without re-training through the use of few-shot task generalization and in-context learning abilities of instruction-tuned language models.

==> macro.tex <==
%%%%
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{array}
\usepackage{arydshln}
\usepackage{multirow}
\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{amsmath}
% \DeclareMathOperator{\max}{max}
\usepackage{graphicx}
\usepackage{makecell}
% \usepackage[utf8x]{inputenc}  % unicode
% \usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{lipsum}  % generates filler text
\usepackage{etoolbox}
\usepackage{comment}
% Math, Images and others
\usepackage{enumitem}
\renewcommand{\UrlFont}{\ttfamily\small}
\usepackage{booktabs}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  
\usepackage{microtype}
\usepackage{csquotes}
\usepackage{bm}
\usepackage{amsmath,amssymb, amsfonts,mathtools}
\usepackage{soul}
\usepackage{adjustbox}
\usepackage[]{todonotes}
% \usepackage[dvipsnames]{xcolor}
\usepackage[capitalize]{cleveref}
\usepackage{hyperref}
\usepackage{appendix}
\usepackage{svg}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}
\BeforeBeginEnvironment{appendices}{\clearpage}

\Crefname{appsec}{appendix}{appendices}

\usepackage{caption}
\usepackage{subcaption}
% commented out as this makes the `enumerate` command require extra arguments which are currently not provided -vilem
% \usepackage{enumerate}
\usepackage{scalerel}
% \usepackage[titilenumbered,ruled,vlined]{algorithm2e}
\usepackage{linguex}
\usepackage{relsize}
\usepackage{array}
\usepackage{booktabs}
\usepackage{array}
\usepackage{makecell}
\usepackage{relsize}
\usepackage{multirow}
\newcommand{\defeq}[0]{\mathrel{\stackrel{\textnormal{\tiny def}}{=}}}
\usepackage[font=small,labelfont=bf]{caption}
% \setlength\titlebox{4.25cm}

\usepackage{cancel}
\usepackage{inconsolata}


% added this macro because it was missing before, taken from seq2class.sty -vilem
\newcommand{\noindentaftertodo}{\noindent}

% Comments: 
\usepackage{todonotes}
% Note that these macros accept optional arguments such as size=\small, bordercolor=red, and so on.  Capitalized versions are inline paragraphs instead of margin notes.
\newcommand{\fixme}[2][]{\todo[color=yellow,size=\scriptsize,fancyline,caption={},#1]{#2}} % to mark stuff that you know is missing or wrong when you write the text
\newcommand{\note}[4][]{\todo[author=#2,color=#3,size=\scriptsize,fancyline,caption={},#1]{#4}} % default note settings, used by macros below.
\newcommand{\mrinmaya}[2][]{\note[#1]{mrinmaya}{green}{#2}\xspace}
\newcommand{\ryan}[2][]{\note[#1]{ryan}{violet!40}{#2}\xspace}
\newcommand{\eleanor}[2][]{\note[#1]{eleanor}{yellow}{#2}\xspace}
\newcommand{\chunshu}[2][]{\note[#1]{chunshu}{teal!20}{#2}\xspace}
\newcommand{\Fixme}[2][]{\note[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Notewho}[3][]{\notewho[inline,#1]{#2}{#3}\noindentaftertodo}
\newcommand{\Ryan}[2][]{\ryan[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Mrinmaya}[2][]{\mrinmaya[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Eleanor}[2][]{\eleanor[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Chunshu}[2][]{\chunshu[inline,#1]{#2}\noindentaftertodo}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\newcommand{\tianyu}[2][]{\note[#1]{tianyu}{babyblue}{#2}\xspace}
\newcommand{\response}[1]{\vspace{3pt}\hrule\vspace{3pt}\textbf{#1:}}

\usepackage[dvipsnames]{xcolor}
\definecolor{mygreen}{HTML}{7FC07F}
\definecolor{myred}{HTML}{DF7F7F}
\definecolor{mygray}{HTML}{BAB7B7}
\definecolor{pine}{HTML}{BCE672}
\definecolor{lotus}{HTML}{E4C6D0}
\definecolor{gold}{HTML}{F2BE45}
\definecolor{bamboo}{HTML}{789262}
\definecolor{jade}{HTML}{3DE1AD}
\definecolor{blueblue}{HTML}{4C8DAE}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\ca}[1]{{\color{BrickRed} #1}}
\newcommand{\cb}[1]{{\color{ForestGreen} #1}}
\newcommand{\cc}[1]{{\color{blueblue} #1}}
\newcommand{\cd}[1]{{\textcolor{gold}{#1}}}
\newcommand{\ce}[1]{{\color{bamboo} #1}}
\newcommand{\cf}[1]{{\color{violet} #1}}


%Eleanor's macros
% Annotation
\usepackage{stmaryrd}
\newcommand{\den}[2]{\left\llbracket\mathrm{#1}\right\rrbracket_{#2}}
\newcommand{\coloredUlEntity}[2]{\textcolor{#1}{\textbf{\underline{#2}}}}
\newcommand{\coloredEntity}[2]{\textcolor{#1}{\textbf{#2}}}
\newcommand{\redEntity}[1]{\coloredEntity{red}{#1}}
\newcommand{\blueEntity}[1]{\coloredEntity{blue}{#1}}
\newcommand{\Verb}[1]{\textcolor{teal}{\textbf{\textit{#1}}}}
\newcommand{\Wrong}[1]{\underline{#1}}
\newcommand{\VerbWrong}[1]{\textcolor{teal}{\textbf{\textit{\underline{#1}}}}}
\newcommand{\Qiao}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\Husband}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\Omit}[1]{$\llbracket$\textbf{#1}$\rrbracket$}
\newcommand{\orangeOmit}[1]{\textcolor{orange}{\Omit{#1}}}
\newcommand{\QiaoOmit}[1]{\textcolor{red}{\Omit{#1}}}
\newcommand{\grayEntity}[1]{\textcolor{gray}{\textbf{#1}}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\Chinese}[1]{\begin{CJK*}{UTF8}{gbsn}{#1}\end{CJK*}}

% Discourse related Math Symbols
\newcommand{\defn}[1]{\textbf{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\constraints}{\bm{\mathcal{C}}}
\newcommand{\constraint}{\mathcal{C}}
\newcommand{\mention}{{\color{blue} m}}
\newcommand{\spans}{\mathsf{span}}
\newcommand{\discourse}{\mathfrak{D}}
\newcommand{\discourseSet}{\mathbb{D}}
\newcommand{\corpus}{\mathfrak{C}}
\newcommand{\vocab}{\mathcal{V}}
\newcommand{\Un}{S}
\newcommand{\UnSet}{\mathbb{S}_n}
\newcommand{\NA}{\mathrm{NA}}
\newcommand{\Cdot}{\boldsymbol{\cdot}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

% BlonD Math Symbols and Functions
\newcommand{\reCat}[1]{\mathcal{R}^{#1}}
\newcommand{\sysCat}{\mathcal{S}}
\newcommand{\category}{\mathbf{C}}
\newcommand{\categories}{\mathbf{C}}
\newcommand{\allcategories}{\mathbf{C}}
\newcommand{\weight}{\mathsf{weight}}
\newcommand{\categorizing}{\mathsf{cat}}
\newcommand{\similarity}{\bm{\mathsf{sim}}}
\newcommand{\countFun}{\bm{\mathsf{count}}}

% Math
\newtheorem{defin}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{myexample}{Example}
\newtheorem{mytransform}{Transform}


% Error Types
\newcommand{\NoError}{\textsc{no error}}
\newcommand{\Document}{\textsc{document}}
\newcommand{\Sentence}{\textsc{sentence}}
\newcommand{\Inconsistency}{\textsc{inconsistency}}
\newcommand{\NamedEntity}{\textsc{named entity}}
\newcommand{\Entity}{\textsc{entity}}
\newcommand{\Tense}{\textsc{tense}}
\newcommand{\Ellipsis}{\textsc{ellipsis}}
\newcommand{\Pronoun}{\textsc{pronoun}}
\newcommand{\Others}{\textsc{other}}
\newcommand{\Ambiguity}{\textsc{ambiguity}}
\newcommand{\DiscourseMarker}{\textsc{dm}}

% Math Symbols of Categories
\newcommand{\entities}{\mathcal{E}}
\newcommand{\verbs}{\mathcal{V}}
\newcommand{\pronouns}{\mathcal{P}}
\newcommand{\dms}{\mathcal{M}}

% keys of Categories
\newcommand{\key}[1]{\texttt{#1}}
% DM: \key{contigency}, \key{temporal}, \key{expansion}, \key{comparison}
% Pronoun: masculine, feminine, neuter, epicene
\newcommand{\Masculine}{\key{masculine}}
\newcommand{\Feminine}{\texttt{feminine}}
\newcommand{\Neuter}{\key{neuter}}
\newcommand{\Epicene}{\key{epicene}}
\newcommand{\he}{\texttt{he/him/his/himself}}
\newcommand{\she}{\texttt{she/her/hers/herself}}
\newcommand{\itt}{\texttt{it/its/itself}}
\newcommand{\they}{\texttt{they/them/their/theirs/themselves}}


% Dataset
\newcommand{\BWB}{$\mathcal{BWB}$}

% MT Systems
\newcommand{\SRC}{\textsc{src}}
\newcommand{\REF}{\textsc{ref}}
\newcommand{\MT}{\textsc{mt}}
\newcommand{\MTa}{\textsc{mta}}
\newcommand{\MTb}{\textsc{mtb}}
\newcommand{\SMT}{\textsc{smt}}
\newcommand{\OMTa}{\textsc{omt-a}}
\newcommand{\OMTb}{\textsc{omt-b}}
\newcommand{\OMTc}{\textsc{omt-c}}
\newcommand{\MTS}{\textsc{mt-s}}
\newcommand{\MTD}{\textsc{mt-d}}
\newcommand{\CADec}{\textsc{cadec}}
\newcommand{\CTX}{\textsc{ctx}}
\newcommand{\PE}{\textsc{pe}}

% MT Metrics
\newcommand{\BLEU}{\textsc{bleu}}
\newcommand{\BlonD}{\textsc{blonde}}
\newcommand{\BlonDp}{\textsc{blonde+}}
\newcommand{\COMET}{\textsc{comet}}
\newcommand{\BERTScore}{\textsc{bert}}
\newcommand{\METEOR}{\textsc{meteor}}
\newcommand{\TER}{\textsc{ter}}
\newcommand{\ROUGEL}{\textsc{rouge-l}}
\newcommand{\CIDEr}{\textsc{CIDEr}}
\newcommand{\LC}{\textsc{lc}}
\newcommand{\RC}{\textsc{rc}}
\newcommand{\APT}{\textsc{apt}}
\newcommand{\DiscoTK}{\textsc{DiscoTK}}
\newcommand{\Skip}{\textsc{skip}}
\newcommand{\Aver}{\textsc{aver}}
\newcommand{\Vector}{\textsc{vector}}
\newcommand{\Greedy}{\textsc{greedy}}


% Evaluation Related
\newcommand{\fluency}{\textsc{fluency}}
\newcommand{\success}{\textsc{succ}}
\newcommand{\adequacy}{\textsc{adequacy}}
\newcommand{\testset}[1]{\textsc{part#1}}
\newcommand{\rater}[1]{\textsc{rater#1}}
\newcommand{\diff}[2]{$\Delta$(#1, #2)}
% Table and Other Shortcuts
\newcommand{\MyIndent}{\hspace{0.5cm}}
\newcommand{\myFontSize}{\scriptsize}
\def\stripzero#1{\expandafter\stripzerohelp#1}
\def\stripzerohelp#1{\ifx 0#1\expandafter\stripzerohelp\else#1\fi}
%\aclfinalcopy % Uncomment this line for the final submission
% \def\aclpaperid{1562} %  Enter the acl Paper ID here
% \authorimg{acl2020-templates/blond-1.png}
% \usepackage[symbol]{footmisc}


%%%%%% MY PACKAGES & NEW COMMANDS
\usepackage{amssymb,graphicx}
\usepackage{tikz}
\usetikzlibrary{fit,calc}
\usepackage{pgfplots}
\usepackage{float}
\restylefloat{table}
\usepackage{booktabs}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\topK}{TopK}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\pairb}[1]{\left( #1 \right)}
\newcommand{\bigO}[1]{\mathcal{O}(#1)}


\newcommand{\xra}[1]{\overset{#1}{\rightsquigarrow}}
\newcommand{\xla}[1]{\overset{#1}{\leftsquigarrow}}

\newcommand{\openm}[0]{\texttt{<m>}}
\newcommand{\closem}[0]{\texttt{<\textbackslash m>}}


% algorithm
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}  % do not also use algorithmic
\algrenewcommand\algorithmicindent{1.0em}%
\renewcommand\algorithmicdo{:}
\renewcommand\algorithmicthen{:}
% renewcommand -> newcommand -vilem
\newcommand{\rightcomment}[1]{{\color{gray} \(\triangleright\){\footnotesize\textit{#1}}}}
\algrenewcommand{\algorithmiccomment}[1]{\hfill \rightcomment{#1}}  % redefines \Comment
% \algrenewcommand{\Comment}[1]{\hfill \rightcomment{#1}} 
\algnewcommand{\LineComment}[1]{\State\rightcomment{#1}}
\algnewcommand{\LinesComment}[1]{\State\rightcomment{\parbox[t]{.95\linewidth-\leftmargin-\widthof{\(\triangleright\) }}{#1}}}
\renewcommand\algorithmicdo{:}
\renewcommand\algorithmicthen{:}
\algrenewcommand\alglinenumber[1]{{\tiny\color{black!50}#1.}\hspace{-2pt}}

\newcommand{\algorithmicfunc}[1]{\textbf{def} {#1}:}
\algdef{SE}[FUNC]{Func}{EndFunc}[1]{\algorithmicfunc{#1}}{}
\makeatletter
\ifthenelse{\equal{\ALG@noend}{t}}%
  {\algtext*{EndFunc}}
  {}%
\makeatother
\usepackage{inconsolata}
% Reference
\usepackage{cleveref}
\crefname{section}{\S}{\S\S}
\Crefname{section}{\S}{\S\S}
\crefname{table}{Tab.}{}
\crefname{figure}{Fig.}{}
\crefname{algorithm}{Alg}{}
\crefname{algorithm}{Alg}{}
\crefname{line}{line}{lines}
\Crefname{line}{Line}{Lines}
\crefname{appendix}{App.}{}
\crefformat{section}{\S#2#1#3}
\crefname{thm}{Theorem}{}
\crefname{prop}{Proposition}{}
\crefname{defin}{Definition}{}
\crefname{lemma}{Lemma}{}
\crefname{cor}{Corollary}{}
\crefname{equation}{}{}

% general formal language theory macros
\newcommand{\alphabet}{{ \Sigma}}
\newcommand{\stackalphabet}{{ \Gamma}}
\newcommand{\oalphabet}{{ \Delta}}
\newcommand{\lang}{{ L}}
\newcommand{\kleene}[1]{{#1^*}}
\newcommand{\kleeneplus}[1]{{#1^+}}
\newcommand{\rankedalphabet}{{ \left(\alphabet, \arity)\right}}
\newcommand{\edge}[3]{{#1 \xrightarrow{#2} #3}}
\newcommand{\regex}{{ \alpha}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\powerset}[1]{2^{#1}}
\newcommand{\binv}[1]{{\left(#1\right)^{-1}}}
\newcommand{\str}{{\boldsymbol{s}}}
\newcommand{\xx}{{\boldsymbol{x}}}
\newcommand{\yy}{{\boldsymbol{y}}}
\newcommand{\zz}{{\boldsymbol{z}}}
% matrices
\newcommand{\bW}{{ \mathbf{W}}}
\newcommand{\bY}{{ \mathbf{Y}}}
\newcommand{\bG}{{ \mathbf{G}}}
\newcommand{\bR}{{ \mathbf{R}}}
\newcommand{\bS}{{ \mathbf{S}}}
\newcommand{\bI}{{ \mathbf{I}}}
\newcommand{\bA}{{ \mathbf{A}}}
\newcommand{\bB}{{ \mathbf{B}}}
\newcommand{\bC}{{ \mathbf{C}}}
\newcommand{\bM}{{ \mathbf{M}}}
\newcommand{\bE}{{ \mathbf{E}}}
\newcommand{\bT}{{ \mathbf{T}}}
\newcommand{\bO}{{ \mathbf{O}}}
\newcommand{\bw}{{ \mathbf{w}}}

% data structures
\newcommand{\queue}{{\textsf{queue}}}
\newcommand{\stack}{{\textsf{stack}}}
\newcommand{\inblock}{{\textsf{in-block}}}

% graphs
\newcommand{\graph}{ \mathcal{G}}
\newcommand{\scc}{ \mathcal{S}}

% semirings
\newcommand{\semiring}{{ \mathcal{W}}}
\newcommand{\semiringtuple}{{\left(\semiringset, \oplus, \otimes, \zero, \one \right)}}
\newcommand{\closedsemiringtuple}{{ \left(\semiringset, \oplus, \otimes, \zero, \one, \kleene{} \right)}}
\newcommand{\semiringset}{{A}}
\newcommand{\zero}{{\textbf{0}}}
\newcommand{\one}{{\textbf{1}}}

%%%%%%%% MT %%%%
\newcommand{\by}{{\bm{y}}}
\newcommand{\bx}{{\bm{x}}}
\newcommand{\bz}{{\bm{z}}}
\newcommand{\bh}{{\bm{h}}}
\newcommand{\BOS}{{\mathrm{BOS}}}
\newcommand{\EOS}{{\mathrm{EOS}}}

%%%%%%%% Latent Variable Decoding %%%%
\newcommand{\LModel}{p_{\bm{\theta}}}
\newcommand{\latent}{z}
\newcommand{\zspace}{\Gamma}
\newcommand{\hyp}{\mathrm{hyp}}
\newcommand{\pos}{{\color{blue} l}}
\newcommand{\state}{{\color{blue} q}}
\newcommand{\reward}{r}
\newcommand{\addReward}{{\color{blue} a}}
\newcommand{\beam}{\bm{B}}
\newcommand{\matchScoreF}{\bm{\mathsf{matchScore}}}
\newcommand{\scoreF}{\bm{\mathsf{score}}}
\newcommand{\rescoreF}{\bm{\mathsf{rescore}}}
\newcommand{\encodeF}{\bm{\mathsf{Encode}}}
\newcommand{\forceF}{\bm{\mathsf{force}}}
\newcommand{\groupF}{\bm{\mathsf{group}}}
\newcommand{\qualityF}{\bm{\mathsf{quality}}}
\newcommand{\stosModelF}{{\color{blue} f}}
\newcommand{\rewardF}{\bm{\mathsf{reward}}}
\newcommand{\startNewScore}{\textsf{startNewScore}}
\newcommand{\concludeNewScore}{\textsf{concludeNewScore}}
\newcommand{\softmax}{\mathsf{softmax}}
\newcommand{\ScoreVectorM}{\bm{\mathsf{ScoreM}}}
\newcommand{\newMention}{\epsilon}
\newcommand{\emptySet}{\bm{\phi}}
% removed as it is not used and is conflicting with the original macro -vilem
% \newcommand{\ref}{r}


% Algo
\newcommand{\beamSearch}{{\color{blue} \text{beamSearch}}}
\newcommand{\decodingFixedM}{{\color{blue} \text{latentVariableDecoding}}}
\newcommand{\copyF}{{\color{blue} \text{copy}}}
\newcommand{\generateF}{{\color{blue} \text{generate}}}
\newcommand{\startF}{{\color{blue} \text{start}}}

% input
% \newcommand{\Input}{}
\newcommand{\maxHypLen}{T}
\newcommand{\maxBeamSize}{b_{max}}
\newcommand{\Input}{\hspace*{\algorithmicindent} \textbf{Input:}}
\newcommand{\Output}{\hspace*{\algorithmicindent} \textbf{Output:}}


\newcommand{\qchild}{{ q'}}
\newcommand{\qparent}{{ q_{\text{P}}}}
\newcommand{\transitions}{{ E}}
\newcommand{\failureexpansion}{{ \overline{\transitions}}}
\newcommand{\initf}{{ \lambda}}
\newcommand{\finalf}{{ \rho}}
\newcommand{\failuref}{{ \phi}}
\newcommand{\wfsa}{{ \mathcal{A}}}
% \newcommand{\expandedwfsa}{{ \wfsa_{\textsc{expanded}}}}
\newcommand{\expandedwfsa}{{ \wfsa_{\textsc{exp}}}}
\newcommand{\wfsatuple}{{ \langle \alphabet, \states, \transitions, \initf, \finalf \rangle}}

==> sections/0_abstract.tex <==
\begin{abstract}

Large language models generate fluent texts and can follow natural language instructions to solve a wide range of tasks without task-specific training. Nevertheless, it is notoriously difficult to control their generation to satisfy the various constraints required by different applications. In this work, we present \method, a controlled text generation framework that incorporates different constraints by conditioning on natural language descriptions and demonstrations of the constraints. In particular, we first extract the underlying constraints of natural texts through a combination of off-the-shelf NLP tools and simple heuristics. We then verbalize the constraints into natural language instructions to form weakly supervised training data. By prepending natural language descriptions of the constraints and a few demonstrations of the input, we fine-tune a pre-trained language model to incorporate various types of constraints. Compared to existing search-based or score-based methods, \method is more flexible to different constraint types and has a much smaller impact on the generation quality and speed because it does not modify the decoding procedure.
Additionally, \method allows the model to adapt to new constraints without re-training through the use of few-shot task generalization and in-context learning abilities of instruction-tuned language models. Code will be available at \url{https://github.com/MichaelZhouwang/InstructCTG}

\end{abstract}



==> sections/1_introduction.tex <==
\section{Introduction}
Large language models (LLMs) pre-trained on web-scale corpora~\citep{gpt,gpt2,gpt3} have demonstrated impressive ability to generate fluent and realistic texts. Yet, many text generation applications require the model to generate texts that not only possess a high degree of naturalness but also adhere to task-specific constraints. For example, a question generation system may require the model to incorporate certain keywords during generation, and a dialog system may be expected to generate responses that are easily understandable and not toxic or biased. Therefore, controlled text generation is an important feature in natural language generation applications.

\begin{figure}[t]
    \centering
    \vspace{-10pt}
     % \imgtrimleftsize{} \imgtrimbottomsize{} \imgtrimrightsize{} \imgtrimtopsize
   \includegraphics[width=0.48\textwidth,trim={0cm 0.1cm 0cm 0.8cm} ,clip]{figures/motivation.pdf}
    \vspace{-6pt}
    \caption{A diagram of the \method framework. The controlled text generation tasks we consider in this work are:  \textsc{lexical}, \textsc{syntax}, \textsc{semantic}, \textsc{style}, and \textsc{length}.\looseness=-1}
    \vspace{-15pt}
    \label{fig:motivation}
\end{figure}

The dominant paradigm for controlled text generation is to incorporate constraints at decoding time. Prior works either include constraints in the search algorithm by modifying beam search~\citep{hokamp-liu-2017-lexically, anderson-etal-2017-guided,post-vilar-2018-fast,lu-etal-2021-neurologic,lu-etal-2022-neurologic} or convert constraints into energy functions (e.g., classifiers) and use them to guide the score-based sampling process, e.g. using Langevin dynamics~\citep{qin2022cold,kumar2022gradient} or diffusion models~\citep{li2022diffusionlm}. 

While effective in guiding the model to incorporate the constraints, existing decoding-time methods for controlled text generation suffer from a number of limitations. First, both search-based and score-based methods modify the output sequence distribution and thus generally result in worse generation quality~\citep{lin-etal-2020-commongen}. Second, existing methods require extra computation and lead to slower generation speed~\citep{post-vilar-2018-fast,li2022diffusionlm}. Third, previous methods are less flexible when dealing with new kinds of constraints or composition of different constraints. Finally, while search-based methods are mostly limited to lexical constraints, score-based methods require training or designing new score functions for new constraints, and need to be carefully tuned in order to achieve a good trade-off between constraint satisfaction and generation quality.
%the relative weights between different constraints and the original language modeling loss

In this paper, we present \method, a new paradigm for controlled generation, which is an alternative to existing methods that modify the decoding procedure of the model. \method is inspired by the recent observations that large pre-trained language models can generalize to various tasks without task-specific training by following natural language descriptions~\citep{zhong-etal-2021-adapting-language, wei2022finetuned,sanh2022multitask} or a few demonstrations of the task~\citep{gpt3,min-etal-2022-metaicl}. By considering controlled text generation as a combination of the text generation task and the task of following certain constraints, \method incorporates constraints by prepending a prompt, which verbalizes the constraints into natural language instructions, to the task-specific inputs. 

In particular, \method is trained in a weakly-supervised fashion on general text corpora by considering a corpus of texts that is generated under various kinds of constraints that are automatically inferred using off-the-shelf NLP tools or simple rules. As a concrete example, in the case of generating a sentence with a length constraint and some keyword constraints, the length is derived by a tokenizer, and a portion of nouns and verbs in the sentence are extracted by a POS tagger and treated as the keywords.
After obtaining the constraints to be imposed for generating a sentence, we verbalize the constraints into a natural language instruction. In this way, we can instruction-tune the model by prepending 
the constraint instruction to the task-specific input following~\citep{wei2022finetuned,sanh2022multitask}. Moreover, to improve the ability of \method to few-shot generalize to unseen constraints without fine-tuning the model, we incorporate meta in-context learning~\citep{min-etal-2022-metaicl} by including a few demonstrations of the constraints in the prefix. Compared to previous decoding-based methods, \method allows the model to understand the constraints before decoding so that it can generate desirable outputs without constrained or score-based decoding, leading to improved generation quality and efficiency. \method is also more flexible with respect to different kinds of constraints and unseen constraints during training. 

To evaluate the effectiveness of \method, we conduct a wide range of experiments with different constraint types including the keywords, syntax, semantic, style and length, by fine-tuning T0~\citep{sanh2022multitask}, an instruction-tuned text-to-text pre-trained model.
Our results show that \method achieves a high level of constraint satisfaction rate that is comparable to state-of-the-art decoding-based methods while producing outputs of superior quality, and is capable of doing so at a significantly faster generation speed. Additionally, \method demonstrates strong generalization abilities in the context of few-shot learning, specifically with regard to the constraints that are unseen during training. This represents a novel and important advancement in comparison to existing methods.

% Current methods for controlled text generation enforce either hard (decoding algorithms) or soft (score-based methods) constraints when searching in the output logits/probability space. However, the model itself is generally unaware of the constraints when doing encoding, attention, etc. This results in decreased generation quality.

% Moreover, most existing methods needs to design/train new algorithms/classifiers for new constraint types. This can be inconvenient (decoding-based method cannot apply to contraint types other than lexical constraints). In addition, these approaches leads to significantly slower generation.

% Recent advances on prompt/instruction learning show that pre-trained models can be fine-tuned to follow task descriptions specified as natural language instructions and achieve good multi-task performance as well as zero-shot task generalization ability. The success of task instruction tuning motivate us to explore \textit{constraint instruction tuning}, where different constraint types are described in natural language and prepend to the input as instructions. 

% In constraint instruction tuning, we first verbalize various constraint types into short natural language descriptions. We then construct weakly(or self?)-supervised training data by annotating the underlying constraint codes of different constraint types for sentences in general text corpora with corresponding off-the-shelf NLP models or toolkits. For example, for lexical constraints and syntax constraints, we use Spacy POS tagger and constituency parser to extract keywords and syntax trees from sentences. Finally, we follow task instruction tuning and fine-tune a task instruction fine-tuned model (e.g., T0) to generate sentences with natural language descriptions of constraints annotated in the previous step.

% To further enable the model to deal with compositions of constraints and unseen constraints, we randomly compose different constraints during fine-tuning and add a meta in-context learning stage after constraint instruction tuning. After meta in-context learning with demonstrations of constraints and compositions of constraints, the model can generalize to unseen compositions of constraints and even new constraint types with a few demonstrations.

% Modeling constraints as natural language instructions has the following advantages:
% \begin{itemize}
% \item The model is able to understand the constraints during the encoding process and pay attention to constraints during decoding. Therefore, the need of perturbation on the decoding search space is alleviated, leading to improved generation quality.
% \item Alleviate the need of tuning the relative weight of generation quality and constraints satisfaction and designing new algorithms or training new classifiers for new constraints. -> less engineering efforts
% \item Significantly improved decoding speed (almost the same with conventional decoding, just need to encode some extra tokens in the encoder, which is parallel).
% \end{itemize}

==> sections/2_relatedwork.tex <==
\section{Related Work}

\paragraph{Neural text generation}
Neural text generation generally involves two stages: learning and decoding. The learning stage models a probability distribution over text sequences, which is typically computed by factorizing the probability of a text sequence into the product of per-token conditional probabilities in left-to-right order. The per-token conditional probabilities are often parameterized with a shared neural network such as a LSTM~\citep{hochreiter1997long} or a Transformer~\citep{transformer}. The parameters of the neural network are typically learned by maximum likelihood estimation with teacher forcing, which feeds observed sequences (i.e. ground-truth samples) back into the neural network after each step. After learning, the decoding stage aims to sample a text sequence from the probability distribution learned in the learning stage. Popular decoding algorithms includes beam search and its variants which are optimized for sample quality and sampling methods such as top-k sampling~\citep{fan2018hierarchical}, nucleus sampling~\citep{holtzman2019curious}, and typical decoding~\citep{meister2022locally}, which are optimized for the quality-diversity trade-off.
%$\by = y_1 y_2 \cdots y_T$ in the language $\lang \subseteq\kleene{\vocab}$ 

\vspace{-2pt}
\paragraph{Controlled text generation}
Conventional decoding algorithms cannot incorporate constraints during generation. Therefore, they can not ensure the output satisfies certain requirements that are important to certain applications. To this end, there exists two distinct lines of research focusing on controlled text generation which focus on constrained search algorithms and score-based sampling methods respectively. 

Constrained search algorithms enforce strict lexical constraints on the outputs by modifying the search space according to the constraints. Constrained beam search (CBS) algorithm~\citep{anderson-etal-2017-guided}, first proposed to track constraint satisfaction using a finite-state machine, encourages the model to fulfill unsatisfied constraints at each step. However, CBS requires the model to maintain a finite-state machine with $2^C$ states (where $C$ is the number of constraints), resulting in significantly increased inference latency. To reduce the runtime overhead of CBS, ~\citet{hokamp-liu-2017-lexically} and ~\citet{post-vilar-2018-fast} introduced grid beam search (GBS) and dynamic beam allocation (DBA). Specifically, GBS reduces inference to linear run-time complexity by forcing the constraint tokens at each time step and grouping together hypotheses based on the number of constraints satisfied. DBA further reduces the dependence on $C$ by fixing the beam size and splitting the beam into subgroups that corresponds to different constraint satisfaction statuses. Finally, \citet{lu-etal-2021-neurologic} recently introduced NeuroLogic decoding, a constrained search algorithm that aims to satisfy rich logic-based lexical constraints expressed in Conjunctive Normal Form (CNF) and extend it to NeuroLogic A$^*$ decoding~\citep{lu-etal-2022-neurologic} by incorporating lookahead heuristics. While existing constrained search algorithms significantly improve the constraint satisfaction rate,  they still lead to slower generation speed and lower fluency and quality because they prune the output distribution space aggressively and thus tend to collapse into globally suboptimal results. Moreover, most constrained search algorithms cannot incorporate constraint types other than lexical constraints.

Score-based sampling methods attempt to incorporate constraints by converting constraints into differentiable score functions. Specifically, score functions for soft constraints such as sentiment control can be implemented as the cross entropy loss of corresponding classifiers. Hard constraints such as lexical constraints can be modeled by a differentiable n-gram matching function~\citep{liu-etal-2022-dont}. With score functions of different constraints, controlled text generation can be achieved by score-based generative models such as Langevin dynamics based models~\citep{song2022langevin,qin2022cold,kumar2022gradient} and diffusion models~\citep{diffusion,li2022diffusionlm} on either logit space or embedding space. Compared to constrained search algorithms, score-based sampling methods are more flexible because they can deal with more diverse constraint types and composition of different constraints. However, score-based sampling methods do not come with constraint satisfaction guarantees and often lead to worse generation quality because the output distribution is modified~\citep{qin2022cold}. Moreover, score-based sampling methods lead to much slower generation speed because multiple score matching steps need to be performed. They also require carefully tuned relative weights between the scores of different constraints and the task-specific loss to achieve a good trade-off between the quality and the constraint satisfaction rate of output texts.

Apart from search-based and score-based methods, \citet{dinu-etal-2019-training} proposed a specialized training method which appends lexical constraints in the input when training the model. Another related work is the CTRL~\citep{keskar2019ctrl} which is pre-trained with structures that naturally co-occur with raw texts and can deal with certain kinds of constraints such as style and domain constraints. \method differs from these approaches because it is generally applicable for different constraint types (as long as we can describe it in natural language) instead of being limited to lexical constraints or constraints that can be converted into classifiers. Also, instead of directly appending raw control codes as in \citet{dinu-etal-2019-training}, \method uses natural language instructions to verbalize, explain, and demonstrate the constraints, which makes use of the emergent abilities of large language models and helps the model generalize to unseen constraints.

\vspace{-3pt}
\paragraph{Instruction-tuning \& In-Context Learning}
Recent advances in LLM pre-training~\citep{gpt3,chowdhery2022palm,zhang2022opt} show that a number of interesting abilities emerge when we scale model size and training FLOPs~\citep{wei2022emergent}. Among the various emergent abilities, one of the most interesting ones is that these models can make use of natural language instructions or a couple of demonstrations to solve various tasks in a zero-shot fashion. While it is originally believed that only very large pre-trained language models are capable of few-shot in-context tuning, some recent work shows that moderate-size pre-trained models can also acquire these abilities by instruction-tuning, which synthesizes fine-tuning data that mimics the way LLMs perform in-context learning. Specifically, \citet{wei2022finetuned} and \citet{sanh2022multitask} show that by multi-task fine-tuning pre-trained text generation models to generate task-specific outputs given a natural language instruction describing the task, the model can learn to generalize to unseen tasks without fine-tuning by prepending a natural language instruction for the new task. \citet{min-etal-2022-metaicl} further propose including a few demonstrations in the instructions so that the model can be fine-tuned to do in-context learning. Our work is also related to previous work on using NLG models for data generartion~\citep{zhou-etal-2020-improving-grammatical, schick-schutze-2021-generating,ye-etal-2022-zerogen}.

==> sections/3_method.tex <==
\section{\method}
To enable flexible, high-quality, and fast controlled text generation, we introduce \textit{Instruction-based Controlled Text Generation} (\method), a prompt-based controlled text generation framework. 
\method verbalizes constraints into natural language descriptions and uses an instruction consisting of the natural language description and a few demonstrations to encourage the model to incorporate the constraints during generation. 
In this section, we describe the data synthesis method, input format, training method, and inference method of \method in detail.

\subsection{Data Collection}
\label{sec:data}
Typically, instruction-tuning requires labeled training data on massive tasks or datasets. However, most publicly available text generation datasets do not have constraint annotations, and crowdsourcing enough constraints-texts pairs for instruction-tuning can be expensive, time-consuming, and also inflexible for new constraints. To this end, we propose a weakly-supervised data synthesis method to synthesize constraints-texts pairs for \method.

The main idea of the data synthesis strategy is to consider various kinds of constraints as ``latent variables'' conditioned on which sentences from general text corpora are generated. Instead of using sophisticated and inefficient algorithms to learn a latent variable model for texts and constraints and then infer the latent constraints for sentences, we opt to use simple rules and off-the-shelf NLP tools corresponding to the definition of the constraints. We here describe the constraints used in the training stage of \method:

\vspace{2pt}
{\bf a) Lexical Constraints:} Similar to previous work on constrained decoding, the lexical constraint requires the model to include certain keywords in the output text. To derive the lexical constraints, we adopt the keyword extraction pipeline used in prior work on keyword-based text generation~\citep{lin-etal-2020-commongen,zhou2021pretraining}. Specifically, given an input text sequence, we use a part-of-speech tagger Spacy\footnote{https://spacy.io/models/en\#en\_core\_web\_sm} and extract all \textit{Verbs}, \textit{Nouns}, and \textit{Proper Nouns} from the sentence and randomly sample a portion of them as keywords. We then lemmatize the extracted keywords so that the model will learn to use the proper form for the keywords.

Moreover, we design a data augmentation method to enable \method to handle more complex requirements such as choosing one keyword from a set of keywords and not including a certain word in the output. Specifically, for each keyword, we use a BERT-based lexical substitution system~\citep{zhou-etal-2019-bert} to generate possible alternatives of the keyword in the context. Then we randomly convert a portion of keyword constraints 
to more complex constraints including (1) choosing a keyword among the extracted ones and their machine-generated substitutes and (2) not including the generated substitutes in the output texts. Since the generated substitutes are all related to the original keyword and suitable for the context, it is reasonable to assume these substitutes are not used because of some ``latent'' constraints. We randomly sample sentences from the C4~\citep{raffel2020exploring} dataset to synthesize keyword constraint-text pairs.
%We quantify the success of following lexical constraints by the percentage of 

\paragraph{b) Syntax Constraints:}
We also consider syntax constraints that require the output text to have certain syntactic structures. We follow \citet{li2022diffusionlm} and consider \textbf{parts-of-speech} constraints and \textbf{syntax tree} constraints as two syntax constraints. Parts-of-speech (POS) constraints are posed as a sequence of POS tags (e.g., \textit{Pronoun Verb Determiner
Noun}) and requires the model to generate a sequence of words of the same length whose POS tags (obtained using the Spacy POS tagger) match the target (e.g., He bought a car). Similarly, syntax tree constraint provides a linearized syntactic parse tree (e.g., (S (NP (PRP $*$)) (VP (VBD $*$) (NP (DT $*$) (NN $*$)))) where $*$ denotes a token) and requires the model to generate a text sequence that matches the constraint when parsed with a pre-trained parser~\citep{kitaev-klein-2018-constituency}. Similar to lexical constraints, we randomly sample sentences from the C4 dataset to synthesize syntax constraint-text pairs.
%We quantify success via word-level exact match.

\paragraph{c) Semantic Constraints:}
To enable fine-grained control on the content/semantics of the output text, we also include three semantic constraints including a {\bf topic/domain constraint}, a {\bf sentiment constraint}, and a {\bf political slant constraint}. Concretely, the topic constraint requires the model to produce texts related to a certain topic such as different scientific fields. Similarly, sentiment constraint and political slant constraint control the sentiment polarity and the political slant of the output texts, respectively. For semantic constraints, we first train a RoBERTa-based~\citep{liu2019roberta} classifier on labeled datasets for different semantic constraints by adding a ``not related'' output class which is associated with random sentences from the C4 dataset. For instance, for sentiment constraint, we train a three-way classifier with sentences of positive and negative sentiment from sentiment-labeled datasets, the Amazon Review dataset~\citep{he2016ups} for sentiment control as positive and negative examples. As for examples for the ``not related'' class, we use sentences from the C4 dataset that are filtered by a two-way classifier trained on the Amazon Review dataset to have no sentiment polarity. To simulate the distribution (population) of sentiment-polarized sentences in web texts, we construct the train set with 90\% random sentences and 5\% sentences of positive and negative sentiment. We then apply the trained classifier on more randomly sampled sentences from C4 and use sentences that are labeled to be of positive/negative sentiment with high confidence to synthesize sentiment constraint-text pairs. 

We use the Amazon Review dataset~\citep{he2016ups} and the Political Slant dataset~\citep{voigt2018rtgender} for the sentiment constraint and political slant constraint respectively and use the M2D2 dataset~\citep{reid2022m2d2}, which contains diverse topics in Wikipedia and ArXiv categories, for topic control\footnote{We do not train the topic classifier and collect data from C4 because the M2D2 dataset is large enough.}. 

\paragraph{d) Style Constraints:}
Apart from controlling keywords, syntax, and content, it is also desirable to control the style of the output texts for more flexible controlled text generation. We follow the survey of \citet{jin-etal-2022-deep} and include various style constraints including the formality, politeness, humor/factual/romance style, biasedness, toxicity, and simplicity of the output texts. Similar to sentiment constraints, we also train a style classifier with a ``no style'' class with random sentences and collect stylized sentences from the C4 dataset to construct style constraint-text pairs. We use Grammarly’s Yahoo Answers Formality Corpus (GYAFC) dataset~\citep{rao-tetreault-2018-dear} for formality constraints, the politeness transfer dataset collected by \citet{madaan-etal-2020-politeness} for politeness control, the FlickrStyle stylized caption
dataset~\citep{gan2017stylenet,li-etal-2018-delete} for style control of humor/factual/romance, the Wiki Neutrality Corpus~\citep{pryzant2020automatically} for biasedness control, the PWKP~\citep{zhu-etal-2010-monolingual} dataset for text simplification, and following the data collection method in \citet{tran-etal-2020-towards} for collecting offensive/non-offensive sentences from the C4 dataset.

\paragraph{e) Length Constraints:}
Finally, we also consider the length constraint which controls the length of the output text. The length constraint is defined to be the number of words (measured using the Moses~\citet{koehn-etal-2007-moses} tokenizer) of the output text. We do not use the number of tokens under the model's tokenizer because the word count is more intuitive to both human users and the language model pre-trained on web texts. We consider interval-based length constraint with an interval of 5, which requires the output text to contain between 5$n$ and 5$(n+1)$ words. We construct length constraint-text pairs using randomly sampled sentences from C4 and the Moses tokenizer.

We synthesize 1 million constraint-text pairs for each category of constraints: lexical, syntax, semantic, style, and length. Training examples for constraint types under the same category are equally allocated (e.g., 500K examples for parts-of-speech and syntax tree constraints each). We also collect dev and test sets with 50K examples for each constraint type with the same method.

% \input{tabs/examples}
\input{tabs/new_examples}

\subsection{Constraint Verbalization}
\label{sec:verbalization}

After obtaining a large set of constraint-text pairs, the next step is to verbalize raw constraints in different formats into natural language instructions because \method training requires text-to-text format. As shown in Table \ref{tab:examples}, for each constraint type, we carefully design natural language templates to convert constraint codes into natural language prompts. Verbalizing constraints has a few benefits. First, explaining the constraints in natural language effectively exploits the prompt-based generation ability of the pre-trained model and makes the constraints more understandable to the model. Second, instruction-tuning with natural language descriptions of the constraints enables zero-shot constraint generalization, enabling the model to handle new constraints that are unseen during training by simply describing them in natural language. Moreover, we design multiple diverse natural language templates for each constraint used for training. In this way, the model can learn to better understand the instructions beyond simple memorization, making it more adaptable to new descriptions for unseen constraints.

\subsection{Constraint Composition}
\label{sec:composition}
Controlled text generation applications often poses a few constraints at the same time when generating the output. To enable \method to handle composition of constraints, we infer the constraint codes for different constraints for a portion of randomly sampled C4 texts and compose the constraints by verbalizing them individually and connecting them with ``and''. For example, for a sentence ``He bought a car'' with both lexical and POS constraints, the final instruction will be ``write something with keywords \textit{buy}, \textit{car} and has a parts-of-speech tag of \textit{Pronoun Verb Determiner
Noun}.'' For each sampled text from C4, we first try to produce constraint codes for as many constraint types as possible and then randomly compose a subset of the constraint codes ranging from 2 to 5 constraints. We keep sample texts from the C4 dataset and get another 1 million training examples which compose 2 to 5 constraints.

\subsection{Extension to Conditional Text Generation}
\label{sec:conditional}
The aforementioned data synthesis pipeline is applicable to unconditional text generation. However, enabling controlled text generation for conditional text generation applications is important for real-world applications. Therefore, we extend the above pipeline to conditional text generation tasks by replacing randomly sampled texts from C4 with the ground-truth output in labeled conditional text generation tasks and compose the original task-specific prompt with the natural language instruction for the constraints\footnote{We only consider lexical constraints for simplicity.}. For example, for a training instance paraphrase generation: ``How far is Earth from Sun; What is the distance between Sun and Earth'', the input with lexical constraint would be: ``Write a paraphrase of How far is Earth from Sun with keywords \textit{distance}''. We consider paraphrase generation and question generation with the Quora Question Paraphrase dataset and the SQUAD question generation dataset~\citep{rajpurkar-etal-2016-squad,du-cardie-2018-harvesting} respectively.
\footnote{\url{https://www.kaggle.com/c/ quora-question-pairs}}

\subsection{Instruction-based Meta In-context Learning}
\label{sec:metaicl}
After data synthesis, we use the combination of instruction-tuning~\citep{wei2022finetuned} and meta in-context learning~\citep{min-etal-2022-metaicl} by connecting the natural language instruction for the constraints and a few (i.e., 5) demonstrations (i.e., constraint instruction-output pairs) of the same constraint or composition of constraints as the input text. To enable the model to do controlled text generation both with and without demonstrations, we leave 50\% of the examples with no demonstrations during training. The model is trained with maximum likelihood estimation and teacher forcing following previous work on pre-training and fine-tuning text-to-text models.

In sum, for a text sequence $\mathbf{X}$ in a general text corpus $\mathbf{D}$, the loss function can be expressed by:
\begin{align}
\mathcal{L} &= - \sum_{\mathbf{X} \in D} {\log{p(\mathbf{X}\, | \theta(\phi (\mathbf{{X}})) ; \beta(\phi(\mathbf{{X}}))}}
\end{align}
\label{eq:plm_loss}
where $\theta, \phi, \beta$ denotes the function mapping a text sequence to the derived constraint or composition of constraints; mapping a constraint code to natural language instructions; and mapping a constraint type to randomly sampled 5 examples in the same constraint type, which are described in Section \ref{sec:data}, \ref{sec:verbalization}, and \ref{sec:metaicl}, respectively. We present more training details in Section \ref{sec:training} and the Appendix.
%where $\theta$ denotes the function mapping a text sequence to its possible ''latent'' constraints, which is described in Section \ref{sec:data}; $\phi$ denotes the function mapping constraint codes to natural language instructions, which is described in Section \ref{sec:verbalization}; and $\beta$ denotes the function mapping constraint types to randomly sampled 5 examples in the same constraint type, which is described in Section \ref{sec:metaicl}.

\subsection{Decoding}
At test time, unlike most previous work that requires complex decoding algorithms, \method can perform controlled text generation without any modification to the decoding process. Specifically, we can simply verbalize the target constraints (either using existing templates for seen constraints or writing a new description for unseen constraints) and optionally provide a few examples for the target constraint types. Then we can simply do a conventional beam search for conditional generation and top-k or top-p sampling for unconditional generation, which is much simpler, faster, and tend to generate higher quality outputs.

==> sections/4_experiments.tex <==
\section{Experiments}
%In this section, we conduct experiments to test the empirical effectiveness of \method. We fine-tune T0~\citep{sanh2022multitask}, an instruction-tuned text-to-text pre-trained model, with \method on a number of constraints described in section \ref{sec:data}. After fine-tuning, we test the performance of the resulting model on both training constraints and constraints that are unseen during training. 

\subsection{Experimental Setup}

\input{tabs/results_seen}


\textbf{Model} We use T0-11B as our base model because it is instruction-tuned on many NLP tasks and thus can better understand and follow new task instructions (e.g., instructions for constrained text generation). T0-11B is initialized from the 11B parameters version of T5+LM~\citep{raffel2020exploring}, which is pre-trained on the C4 dataset with the text infilling objective, and instruction-tuned on a collection of various NLP datasets.

\textbf{Training}
\label{sec:training}
Our model is trained on the mixture of training constraint types illustrated in Table \ref{tab:examples}. We reserve one semantic constraint (political slant) and two style constraints (humor and politeness) as unseen constraints, which are used for evaluating the few-shot constraint generalization ability of \method, and train the model on all other constraints. Following \citet{raffel2020exploring}, we assemble our multi-constraints training mixture by combining and shuffling all examples from all training constraints. We train our model with the Adam~\citep{kingma2014adam} optimizer for 100K steps with a learning rate of 1e-4, a batch size of 1024 text pairs, a dropout rate of 0.1, and a learning rate warmup of 8K steps. Similar to \citet{sanh2022multitask}, we perform checkpoint selection by choosing the checkpoint with the highest constraint satisfaction rate on the validation splits of datasets of training constraints. This enables us to measure the true ability of \method to generalize to constraints that are unseen during training.


\textbf{Evaluation}
We use constraint satisfaction rate and fluency as evaluation metrics to compare the performance of models on controlled text generation. The constraint satisfaction rate is evaluated as the percentage of constraints satisfied by the output text for lexical constraint, word-level exact match for parts-of-speech constraint, F1 score for syntax tree constraint, and sample-level success rate for length constraint. For semantic constraints and style constraints, we train a RoBERTa-based classifier to evaluate the satisfaction rate following previous work on text style transfer~\citep{xu-etal-2018-unpaired}. For fluency metric, we use the perplexity of the generated text under OPT-30B, a powerful language model trained on large-scale web text~\citep{zhang2022opt}.

\textbf{Baselines}
We compare \method with both constrained search algorithms and score-based controlled generative models which are detailed below.

\textbf{Dynamic Beam Allocation~\citep{post-vilar-2018-fast}.} DBA is the most popular constrained search algorithm for lexical constrained text generation. It tracks constraint satisfaction status using a finite-state machine and encourages the model to fulfill unsatisfied constraints at each step.

\textbf{NeuroLogic Decoding~\citep{lu-etal-2021-neurologic}.} This method is one of the state-of-the-art constrained search algorithms. NeuroLogic decoding is able to fulfill rich logic-based lexical constraints by using two prefix tries to track unsatisfied positive constraints and satisfied negative constraints.

\textbf{COLD Decoding~\citep{qin2022cold}.} COLD decoding is an energy-based  constrained generation method that incorporates various kinds of constraints as energy functions and then performs through gradient-based sampling with Langevin dynamics in the logits space.

\textbf{Diffusion-LM~\citep{li2022diffusionlm}} This method is a score-based diffusion model that iteratively denoises a sequence of noises into word embeddings and incorporates differentiable constraints by considering them as a part of score functions.

\input{tabs/results_unseen}


\textbf{Constraint-specific Fine-tuning (CFT).} We fine-tune the model on constraint (without verbalization)-text pair for each constraint type. This method is considered as an oracle in \citep{li2022diffusionlm} and is a naive baseline of \method.

To ensure fair comparison, for CBS and NeuroLogic decoding, we fine-tune the pre-trained T0-11B model on the target sentences used for \method training with the unconditional text generation objective since they do not require constraint-specific training. For COLD decoding, we use GPT-J as the backbone model because it requires a decoder-only language model for generation. For Diffusion-LM, we initialize the transformer model with T0-11B parameters and train it on the same unlabeled data that is used for \method training. We also train a model with the same configuration as described in \citet{li2022diffusionlm} with the same data but found it substantially underperforms our implementation. For the CFT baseline, we fine-tune T0-11B on the corresponding datasets for each constraint type.


\subsection{Results on Seen Constraints}

We first present the performance of \method on seen constraints in Table \ref{tab:results_seen}. We can see that \method achieves a comparable or better constraint satisfaction rate compared to state-of-the-art controlled text generation methods while generating much more fluent texts. This suggests that exploiting LLMs and prompt-based methods can be a compelling alternative future direction.

\method is also more efficient in terms of inference latency because it does not modify the decoding procedure of the model and the increased input length caused by the instructions can be handled in parallel, making it almost as fast as conventional generation. For comparison, \method is over 4$\times$ faster than NeuroLogic decoding, a strong search-based algorithm, and over 40$\times$ faster than Diffusion-LM, the state-of-the-art score-based controlled generation method. This confirms the practical advantages of \method over existing decoding-time methods for controlled text generation.

\subsection{Results on Unseen Constraints}

We also evaluate the performance of \method with a few demonstrations of constraints that are unseen during training. This is a unique feature of \method since existing search-based algorithms are only capable of lexical constraints and score-based methods require score functions trained on the train set of the target constraint. We present the results in Table \ref{tab:results_unseen}, where we combine the few-shot performance of \method with the supervised results of existing methods. We find that despite only a few demonstrations and no update to the model, \method achieves a higher constraint satisfaction rate and better output quality compared to score-based methods which use score functions trained on the training data for the constraints. Moreover, \method also performs competitively with CFT, an oracle baseline that fine-tunes the model on the unseen constraints. This shows that \method has strong few-shot constraint generalization ability, allowing the model to handle new constraints by only writing a description and a few examples of them. This can be an important feature for real-world natural language generation applications which need to meet ever-changing constraints according to new requirements.

\input{tabs/results_conditional}


We also conduct an analysis of the in-domain and the out-domain generalization ability of \method. For in-domain tests, we test InstructCTG and the CFT baseline, which are both training on length bins less than 60 words, on length bins over 60 words. We find that CFT’s success rate drops from 100\% to 91\% when increasing the length bin to 100-105 words while InstructCTG’s success rate only drops to 97\%.

For out-domain test, we compare a variant of InstructCTG which is trained on mixture of lexical, syntax, content, and style constraints but is not trained on length constraint, and the original T0-11B model, on the length constraint task. We find that InstructCTG results in 82\% success rate without demonstrations, and 88\% success rate with 5 demonstrations. In contrast, T0-11B only results in 65\% success rate. This confirms that InstructCTG helps generalize on out-domain unseen constraints, and its ability to understand demonstrations plays an important role, which is in line with findings in Table \ref{tab:results_unseen}.

\subsection{Analysis}

\begin{figure}
    \centering
    \vspace{-2pt}
     % \imgtrimleftsize{} \imgtrimbottomsize{} \imgtrimrightsize{} \imgtrimtopsize
   \includegraphics[width=0.3\textwidth,trim={0cm 0.1cm 0cm 1.2cm} ,clip]{figures/constraint_composition.pdf}
    \caption{Results on composition of multiple constraints. The performance is measured by first normalizing \success \ and \fluency \ with the averaged single constraint performance and then calculating the average. For score-based baselines, the relative weights are tuned with random search.}
    \label{fig:constraint_composition}
    \vspace{-0.5cm}
\end{figure}

\textbf{Ablation Study}
We first ablate different design choices of \method to see their relative importance. The results are shown in Table \ref{tab:results_seen} and \ref{tab:results_unseen}. We find that training the model without verbalizing constraint codes into natural language instructions leads to a substantial performance drop, especially on unseen constraints. We think this is because training on verbalized constraint instructions encourages the model to understand the meaning of instructions, thus better generalizing to instructions for new constraints. Using multiple templates for verbalization also marginally improves the performance. We also find that meta in-context learning helps the model generalize to unseen tasks, showing that the model successfully learns to understand the examples of new constraints provided as contexts. We also find that training with multiple constraints at the same time leads to improved performance. In addition, we test different numbers (1, 2, 5, and 10) of demonstrations and find that 5 demonstrations is a good performance-efficiency trade-off.

\textbf{Results on Conditional Generation Tasks}

We then test the performance of \method on conditional natural language generation tasks which are more practical. Therefore, we further fine-tune our model on two conditional text generation tasks and lexical constraint using \method following the procedure described in section \ref{sec:conditional}. The results are shown in Table \ref{tab:results_conditional}. We can see that \method achieves a comparable constraint satisfaction rate compared to state-of-the-art controlled generation methods while leading to substantial improvement in task-specific metrics. This confirms the effectiveness of \method on conditional text generation tasks.

\textbf{Results on Composition of Constraints}
\label{sec:compose_eval}
We also analyze the performance of \method on composition of constraints. The results are shown in Figure \ref{fig:constraint_composition}. We find that \method is much more robust to composition of constraints while also alleviating the need of searching relative weights. This demonstrates the potential of \method to handle multiple constraints at the same time.

==> sections/5_conclusion.tex <==
\section{Discussion}

Finally, we discuss the role of controlled text generation and \method in the era of LLMs such as ChatGPT. 

\paragraph{Is ChatGPT controllable?} First, we experiment with ChatGPT on the considered control codes by reusing the instruction templates. We find that ChatGPT achieves state-of-the-art success rate on the lexical constraint (i.e., 99.3\% lexical coverage on CommonGEN) with minimal prompt engineering and no temperature sweeping. It also achieves competitive performance on semantic constraints. However, for style constraints and length constraints, ChatGPT underperforms \method by a non-neglieable margin. This is kind of surprising because we thought length constraint instructions should be easy to understand. ChatGPT is falling short on syntax constraints. We believe this is because syntax control codes are more complex. This is in line with our experience in prompting ChatGPT: it is often non-trivial to force ChatGPT to follow specified output formats.

\paragraph{How can we make LLMs more controllable?} 
We then describe a possible way to fine-tune LLMs such as LLAMA~\citep{touvron2023llama} so that they can be more controllable when following instructions. We first examine Alpaca~\citep{alpaca} and find that there is almost no instruction containing formatting instructions such as the length of the outputs and how the outputs should be parsed. To this end, we believe it is feasible to extend \method by using ChatGPT to infer formatting instructions for the outputs in instruction data such as Alpaca, and then augment the data with synthesized formatting instructions and then fine-tune the LLM. We leave this for future work.


\section{Conclusion}

In this work, we introduce \method, a new framework for controlled text generation which exploit the instruction following ability of large language models instead of modifying the decoding procedure of the model. \method achieves better generation quality compared to state-of-the-art controlled generation methods while maintaining competitive constraint satisfaction rates. \method also shows strong few-shot generalization ability on unseen constraints, conditional natural language generation tasks, and composition of multiple constraints. These results indicates prompt-based constrained generation is a promising alternative paradigm compared to existing decoding-time methods for controlled text generation.
